Minimizing Queue Length Regret for Arbitrarily Varying Channels

We consider an online channel scheduling problem for a single transmitter-receiver pair equipped with $N$ arbitrarily varying wireless channels. The transmission rates of the channels might be non-stationary and could be controlled by an oblivious adversary. At every slot, incoming data arrives at an infinite-capacity data queue located at the transmitter. A scheduler, which is oblivious to the current channel rates, selects one of the $N$ channels for transmission. At the end of the slot, the scheduler only gets to know the transmission rate of the selected channel. The objective is to minimize the queue length regret, defined as the difference between the queue length at some time $T$ achieved by an online policy and the queue length obtained by always transmitting over the single best channel in hindsight. We propose a weakly adaptive Multi-Armed Bandit (MAB) algorithm for minimizing the queue length regret in this setup. Unlike previous works, we do not make any stability assumptions about the queue or the arrival process. Hence, our result holds even when the queueing process is unstable. Our main observation is that the queue length regret can be upper bounded by the regret of a MAB policy that competes against the best channel in hindsight uniformly over all sub-intervals of $[T]$. As a technical contribution of independent interest, we then propose a weakly adaptive adversarial MAB policy which achieves $\tilde{O}(\sqrt{N}T^{\frac{3}{4}})$ regret with high probability, implying the same bound for queue length regret.

==> networks.tex <==
\section{Extension to Queueing Networks} \label{network}
Since our policy is oblivious to the arrival process or the queue lengths, it can be readily extended to the network setting. 
Consider an arbitrary network $\mathcal{G}(V,E)$ with a fixed routing policy. We are concerned with only the dynamic channel assignment problem at each node. A node may receive packets from exogenous arrivals to the network or from the departed packets from the other nodes in the network. Our performance measure is the worst-case queue-length regret in the network, defined as follows:
\begin{eqnarray*}
	R_{\mathcal{G}}(T) \equiv \max_{v\in V}R_{Q,v}(T),
\end{eqnarray*}
where $R_{Q,v}$ is the queue length regret of the node $v \in V$ in the network. In particular, the benchmark for the above metric is the joint best fixed channel assignment for all nodes in the network.  


Note that any other related metrics such as the sum of queue-length regret can also be considered similarly.   
